Joint tone mapping and denoising of thermal infrared images via multi-scale Retinex and multi-task learning

Cameras digitize real-world scenes as pixel intensity values with a limited value range given by the available bits per pixel (bpp). High Dynamic Range (HDR) cameras capture those luminance values in higher resolution through an increase in the number of bpp. Most displays, however, are limited to 8 bpp. Naive HDR compression methods lead to a loss of the rich information contained in those HDR images. In this paper, tone mapping algorithms for thermal infrared images with 16 bpp are investigated that can preserve this information. An optimized multi-scale Retinex algorithm sets the baseline. This algorithm is then approximated with a deep learning approach based on the popular U-Net architecture. The remaining noise in the images after tone mapping is reduced implicitly by utilizing a self-supervised deep learning approach that can be jointly trained with the tone mapping approach in a multi-task learning scheme. Further discussions are provided on denoising and deflickering for thermal infrared video enhancement in the context of tone mapping. Extensive experiments on the public FLIR ADAS Dataset prove the effectiveness of our proposed method in comparison with the state-of-the-art.

==> Joint tone mapping and denoising of thermal infrared images via multi-scale Retinex and multi-task learning/abbreviations/abbreviations.tex <==
%\addsec*{Abbreviations}
\begin{acronym}
\acro{HVS}[HVS]{Human Visual System}
\acro{HDR}[HDR]{High Dynamic Range}
\acro{bpp}[bpp]{bits per pixel}
\acro{LDR}[LDR]{Low Dynamic Range}
\acro{TMO}[TMO]{Tone Mapping Operator}
\acro{VIS}[VIS]{Visual-Optical}
\acro{TIR}[TIR]{Thermal Infrared}
\acro{SSIM}{Structural Similarity}
\acro{TMQI}{Tone Mapping Quality Index}
\acro{NSS}{Natural Scene Statistics}
\acro{MWIR}{Medium Wavelength Infrared}
\acro{LWIR}{Long Wavelength Infrared}
\acro{fps}{frames per second}
\acro{CNN}{Convolutional Neural Network}
\acro{DCNN}{Deep Convolutional Neural Network}
\acro{MSE}{Mean Square Error}
\acro{MAE}{Mean Absolute Error}
\acro{MS-SSIM}{Multi-Scale Structural Similarity}
\acro{GAN}{Generative Adversarial Network}
\acro{CAN}{Context Aggregation Network}
\acro{GPU}{Graphics Processing Unit}
\acro{VCN}{Volumetric Correspondence Network}
\acro{MS COCO}{Microsoft Common Objects in Context}
\acro{CLAHE}{Contrast Limited Adaptive Histogram Equalization}
\acro{AHE}{Adaptive Histogram Equalization}
\acro{HE}{Histogram Equalization}
\acro{ODM}{Object Detection Measure}
\acro{mAP}{mean Average Precision}
\acro{CGF}{Conditional Gaussian Filter}
\acro{GT}[GT]{Ground Truth}
\acro{MSR}[MSR]{Multi-Scale Retinex}
\acro{SCB}[SCB]{Simplest Color Balance}
\acro{ML}{Machine Learning}
\end{acronym}

==> Joint tone mapping and denoising of thermal infrared images via multi-scale Retinex and multi-task learning/tables/Comparison_CAN_UNet_without_Realtime_TMO.tex <==
\begin{table}[ht]
    \caption{Comparison between the FLIR \ac{TMO}, our optimized MSR and our deep learning-based approximation using the CAN and the U-Net architecture. Both methods can be approximated according to the measures. Mimicking the optimized \ac{MSR} works slightly better according to the \ac{TMQI}.}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{rcccccc}
    \multicolumn{1}{c}{\textbf{}}                    & \textbf{FLIR~\cite{FLIR_dataset}}    & \textbf{\begin{tabular}[c]{@{}c@{}}CAN\\FLIR\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}U-Net\\FLIR\end{tabular}}    & \textbf{\begin{tabular}[c]{@{}c@{}}Optimized \\MSR\end{tabular}}   & \textbf{\begin{tabular}[c]{@{}c@{}}CAN\\Optimized\\MSR\end{tabular}}  & \textbf{\begin{tabular}[c]{@{}c@{}}U-Net\\Optimized\\MSR\end{tabular}}\\ \cline{2-7} 
    \multicolumn{1}{r|}{TMQI$\uparrow$}   & \multicolumn{1}{c|}{\textbf{0.951}} & \multicolumn{1}{c|}{0.939} & \multicolumn{1}{c|}{0.917} & \multicolumn{1}{c|}{0.923}    & \multicolumn{1}{c|}{0.926}  & \multicolumn{1}{c|}{0.933} \\ \cline{2-7} 
    \multicolumn{1}{r|}{Underexposure$\downarrow$}  & \multicolumn{1}{c|}{0.535}  & \multicolumn{1}{c|}{0.0112} & \multicolumn{1}{c|}{\textbf{0.0088}} & \multicolumn{1}{c|}{1.803}     & \multicolumn{1}{c|}{0.372}  & \multicolumn{1}{c|}{0.334} \\ \cline{2-7} 
    \multicolumn{1}{r|}{Overexposure$\downarrow$}   & \multicolumn{1}{c|}{0.899} & \multicolumn{1}{c|}{0.0375} & \multicolumn{1}{c|}{\textbf{0.0025}} & \multicolumn{1}{c|}{1.176}     & \multicolumn{1}{c|}{0.749}  & \multicolumn{1}{c|}{0.494} \\ \cline{2-7} 
    \multicolumn{1}{r|}{Loss of Global Contrast$\downarrow$}     & \multicolumn{1}{c|}{-0.162} & \multicolumn{1}{c|}{-0.100} & \multicolumn{1}{c|}{-0.0948} & \multicolumn{1}{c|}{\textbf{-0.202}}    & \multicolumn{1}{c|}{-0.168}   & \multicolumn{1}{c|}{-0.176} \\ \cline{2-7} 
    \multicolumn{1}{r|}{Loss of Local Contrast$\downarrow$}      & \multicolumn{1}{c|}{-0.0417} & \multicolumn{1}{c|}{-0.0425} & \multicolumn{1}{c|}{\textbf{-0.0482}} & \multicolumn{1}{c|}{-0.0447}   & \multicolumn{1}{c|}{-0.0444}   & \multicolumn{1}{c|}{-0.0474} \\ \cline{2-7} 
    \multicolumn{1}{r|}{Noise Visibility$\downarrow$}            & \multicolumn{1}{c|}{-}  & \multicolumn{1}{c|}{\textbf{27.66}} & \multicolumn{1}{c|}{27.68} & \multicolumn{1}{c|}{30.67}      & \multicolumn{1}{c|}{30.37}   & \multicolumn{1}{c|}{30.61} \\ \cline{2-7} 
    \multicolumn{1}{r|}{Global Temporal Incoherence$\downarrow$} & \multicolumn{1}{c|}{$1.7\text{e}^{-4}$}  & \multicolumn{1}{c|}{$1\text{e}^{-3}$} & \multicolumn{1}{c|}{$1.9\text{e}^{-3}$} & \multicolumn{1}{c|}{\textbf{$\mathbf{2e^{-5}}$}}     & \multicolumn{1}{c|}{$1.2\text{e}^{-3}$}  & \multicolumn{1}{c|}{$2.5\text{e}^{-4}$} \\ \cline{2-7} 
    \multicolumn{1}{r|}{Local Temporal Incoherence$\downarrow$}  & \multicolumn{1}{c|}{0.0048} & \multicolumn{1}{c|}{0.0014} & \multicolumn{1}{c|}{\textbf{0.0012}} & \multicolumn{1}{c|}{0.025}       & \multicolumn{1}{c|}{0.0191}   & \multicolumn{1}{c|}{0.0186} \\ \cline{2-7} 
    \end{tabular}
    }
    \label{tab:Comparison_CAN_UNet}
\end{table}

==> Joint tone mapping and denoising of thermal infrared images via multi-scale Retinex and multi-task learning/tables/Current_baseline.tex <==


\begin{table}[ht]
\caption{Quantitative evaluation comparing different TMOs to form the current baseline.}
\begin{tabular}{rcccc}
    \multicolumn{1}{c}{\textbf{}}                    & \textbf{FLIR~\cite{FLIR_dataset}}                          & \textbf{Realtime TMO~\cite{Eilertsen2015}}          & \textbf{\ac{CGF}~\cite{Haibo_conditional_filtering_MSR}}   & \textbf{\ac{MSR}~\cite{Petro2014}} \\ \cline{2-5} 
    \multicolumn{1}{r|}{TMQI $\uparrow$}                        & \multicolumn{1}{c|}{\textbf{0.951}}   & \multicolumn{1}{c|}{0.809}  & \multicolumn{1}{c|}{0.850}   & \multicolumn{1}{c|}{0.866}\\ \cline{2-5} 
    \multicolumn{1}{r|}{Underexposure $\downarrow$}               & \multicolumn{1}{c|}{\textbf{0.535}}    & \multicolumn{1}{c|}{0.755}  & \multicolumn{1}{c|}{2.842}   & \multicolumn{1}{c|}{1.191}    \\ \cline{2-5} 
    \multicolumn{1}{r|}{Overexposure $\downarrow$}                & \multicolumn{1}{c|}{0.899}    & \multicolumn{1}{c|}{1.628}  & \multicolumn{1}{c|}{\textbf{0.030}}  & \multicolumn{1}{c|}{1.578}   \\ \cline{2-5} 
    \multicolumn{1}{r|}{Loss of Global Contrast $\downarrow$}     & \multicolumn{1}{c|}{\textbf{-0.162}}   & \multicolumn{1}{c|}{-0.123} & \multicolumn{1}{c|}{-0.084}  & \multicolumn{1}{c|}{-0.148}  \\ \cline{2-5} 
    \multicolumn{1}{r|}{Loss of Local Contrast $\downarrow$}      & \multicolumn{1}{c|}{\textbf{-0.0417}} & \multicolumn{1}{c|}{-0.0236} & \multicolumn{1}{c|}{-0.022}  & \multicolumn{1}{c|}{-0.027}  \\ \cline{2-5} 
    \multicolumn{1}{r|}{Noise Visibility $\downarrow$}            & \multicolumn{1}{c|}{-}                 & \multicolumn{1}{c|}{30.77}   & \multicolumn{1}{c|}{30.04}  & \multicolumn{1}{c|}{\textbf{28.79}}  \\ \cline{2-5} 
    \multicolumn{1}{r|}{Global Temporal Incoherence $\downarrow$} & \multicolumn{1}{c|}{$1.7\text{e}^{-4}$}  & \multicolumn{1}{c|}{$3.7\text{e}^{-4}$} &
    \multicolumn{1}{c|}{$\mathbf{2.8e^{-5}}$} &
    \multicolumn{1}{c|}{$2.7\text{e}^{-4}$} \\ \cline{2-5} 
    \multicolumn{1}{r|}{Local Temporal Incoherence $\downarrow$}  & \multicolumn{1}{c|}{\textbf{0.0048}}  & \multicolumn{1}{c|}{0.0157} & \multicolumn{1}{c|}{0.0088}    & \multicolumn{1}{c|}{0.0394} \\ \cline{2-5} 

\end{tabular}
\label{tab:current_baseline}
\end{table}


% \begin{table}[ht]
% \begin{tabular}{rcccc}
%     \multicolumn{1}{c}{\textbf{}}                    & \textbf{FLIR}                          & \textbf{Realtime TMO}          & \textbf{Retinex}             & \textbf{L1L0 TMO}                   \\ \cline{2-5} 
%     \multicolumn{1}{r|}{TMQI $\uparrow$}                        & \multicolumn{1}{c|}{\textbf{0.951}}   & \multicolumn{1}{c|}{0.809}     & \multicolumn{1}{c|}{0.809}   & \multicolumn{1}{c|}{0.761}          \\ \cline{2-5} 
%     \multicolumn{1}{r|}{Underexposure $\downarrow$}               & \multicolumn{1}{c|}{\textbf{0.535}}    & \multicolumn{1}{c|}{0.755}    & \multicolumn{1}{c|}{1.19}    & \multicolumn{1}{c|}{0.81}           \\ \cline{2-5} 
%     \multicolumn{1}{r|}{Overexposure $\downarrow$}                & \multicolumn{1}{c|}{\textbf{0.899}}    & \multicolumn{1}{c|}{1.628}    & \multicolumn{1}{c|}{1.58}    & \multicolumn{1}{c|}{2.2037}         \\ \cline{2-5} 
%     \multicolumn{1}{r|}{Loss of Global Contrast $\downarrow$}     & \multicolumn{1}{c|}{\textbf{-0.162}}   & \multicolumn{1}{c|}{-0.123}   & \multicolumn{1}{c|}{-0.148}  & \multicolumn{1}{c|}{-0.044}         \\ \cline{2-5} 
%     \multicolumn{1}{r|}{Loss of Local Contrast $\downarrow$}      & \multicolumn{1}{c|}{\textbf{-0.0417}} & \multicolumn{1}{c|}{-0.0236}   & \multicolumn{1}{c|}{-0.027}  & \multicolumn{1}{c|}{-0.0078}        \\ \cline{2-5} 
%     \multicolumn{1}{r|}{Noise Visibility $\downarrow$}            & \multicolumn{1}{c|}{-}                 & \multicolumn{1}{c|}{30.77}     & \multicolumn{1}{c|}{28.79}   & \multicolumn{1}{c|}{\textbf{27.47}} \\ \cline{2-5} 
%     \multicolumn{1}{r|}{Global Temporal Incoherence $\downarrow$} & \multicolumn{1}{c|}{\textbf{0.000170}}  & \multicolumn{1}{c|}{0.000365} & \multicolumn{1}{c|}{0.00027} & \multicolumn{1}{c|}{0.0002}         \\ \cline{2-5} 
%     \multicolumn{1}{r|}{Local Temporal Incoherence $\downarrow$}  & \multicolumn{1}{c|}{\textbf{0.00481}}  & \multicolumn{1}{c|}{0.0157}   & \multicolumn{1}{c|}{0.0394}  & \multicolumn{1}{c|}{0.0056}         \\ \cline{2-5} 
%     \multicolumn{1}{r|}{Sharpness $\uparrow$}                   & \multicolumn{1}{c|}{\textbf{1161}}     & \multicolumn{1}{c|}{741}       & \multicolumn{1}{c|}{1130}    & \multicolumn{1}{c|}{85}             \\ \cline{2-5} 
% \end{tabular}
% \caption{Comparison between different TMO`s to form the current baseline}
% \label{tab:current_baseline}
% \end{table}

==> Joint tone mapping and denoising of thermal infrared images via multi-scale Retinex and multi-task learning/tables/Denoising_and_Deflickering_noNormDeflicker_2.tex <==
\begin{table}[ht]
    \caption{Quantitative evaluation of the self-supervised denoising method and denoising with deflickering. The considered denoising approach is first evaluated as post-processing after the approximation of tone mapping. Then, joint training is done with implicit denoising and deflickering. We use Noisy-As-Clean as denoising method in the joint training. Joint TMO+denoising+deflickering performs best according to the measures.}
    \centering
    %\resizebox{\textwidth}{!}{
    \begin{tabular}{rcccc}
    \multicolumn{1}{c}{\textbf{}}                    & \textbf{\begin{tabular}[c]{@{}c@{}}Optimized\\MSR\end{tabular}}    & \textbf{\begin{tabular}[c]{@{}c@{}}Noisy-As-Clean\\denoising as\\post-processing\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Joint TMO\\+denoising\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Joint TMO\\+denoising\\+deflickering\end{tabular}} \\ \cline{2-5} 
    \multicolumn{1}{r|}{TMQI$\uparrow$}                        & \multicolumn{1}{c|}{0.923}  & \multicolumn{1}{c|}{\textbf{0.937}}                                                 & \multicolumn{1}{c|}{\textbf{0.937}}                                         & \multicolumn{1}{c|}{0.934}                                                      \\ \cline{2-5} 
    \multicolumn{1}{r|}{Underexposure$\downarrow$}               & \multicolumn{1}{c|}{1.803}                                                & \multicolumn{1}{c|}{\textbf{0.430}}                                               & \multicolumn{1}{c|}{0.460}                                            & \multicolumn{1}{c|}{1.330}                                           \\ \cline{2-5} 
    \multicolumn{1}{r|}{Overexposure$\downarrow$}                & \multicolumn{1}{c|}{1.176}                                              & \multicolumn{1}{c|}{0.439}                                     & \multicolumn{1}{c|}{\textbf{0.188}}                     & \multicolumn{1}{c|}{1.110}                                                     \\ \cline{2-5} 
    \multicolumn{1}{r|}{Loss of Global Contrast$\downarrow$}     & \multicolumn{1}{c|}{\textbf{-0.202}}        & \multicolumn{1}{c|}{-0.145}                                   & \multicolumn{1}{c|}{-0.133}                                 & \multicolumn{1}{c|}{-0.152}                                                     \\ \cline{2-5} 
    \multicolumn{1}{r|}{Loss of Local Contrast$\downarrow$}      & \multicolumn{1}{c|}{\textbf{-0.044}}        & \multicolumn{1}{c|}{-0.034}                           & \multicolumn{1}{c|}{-0.033}                                                   & \multicolumn{1}{c|}{-0.031}                                                    \\ \cline{2-5} 
    \multicolumn{1}{r|}{Noise Visibility$\downarrow$}            & \multicolumn{1}{c|}{30.67}               & \multicolumn{1}{c|}{26.52}                                              & \multicolumn{1}{c|}{\textbf{25.97}}                                           & \multicolumn{1}{c|}{26.49}                                                      \\ \cline{2-5} 
    \multicolumn{1}{r|}{Global Temporal Incoherence$\downarrow$} & \multicolumn{1}{c|}{$2\text{e}^{-5}$}      & \multicolumn{1}{c|}{$2.4\text{e}^{-4}$}                                     & \multicolumn{1}{c|}{$8.6\text{e}^{-4}$}                                       & \multicolumn{1}{c|}{\textbf{$\mathbf{5.7e^{-6}}$}}                                                    \\ \cline{2-5} 
    \multicolumn{1}{r|}{Local Temporal Incoherence$\downarrow$}  & \multicolumn{1}{c|}{0.025}   & \multicolumn{1}{c|}{0.0229}                                      & \multicolumn{1}{c|}{\textbf{0.0207}}                                     & \multicolumn{1}{c|}{0.0258}                                                     \\ \cline{2-5} 
    \end{tabular}
   % }
    \label{tab:Denoising_and_Deflickering}
\end{table}

==> Joint tone mapping and denoising of thermal infrared images via multi-scale Retinex and multi-task learning/tables/Final_Comparison.tex <==
\begin{table}[ht]
    \caption{Comparison between the state-of-the-art, our optimized \ac{MSR} and our deep learning-based approach with joint denoising and deflickering called \emph{learned MSR}. The performance improvement compared to the baseline \ac{MSR}~\cite{Petro2014} is notable in multiple measures with the \ac{TMQI} and the noise visibility being the most important ones. The other Retinex-based approach \ac{CGF} is outperformed, too.}
    \centering
  %  \resizebox{\textwidth}{!}{
    \begin{tabular}{rcccccc}
    \multicolumn{1}{c}{\textbf{}}   & \textbf{FLIR~\cite{FLIR_dataset}} & \textbf{\begin{tabular}[c]{@{}c@{}}Realtime~\cite{Eilertsen2015}\\TMO\end{tabular}} & \textbf{CGF~\cite{Haibo_conditional_filtering_MSR}} & \textbf{MSR~\cite{Petro2014}} & \textbf{\begin{tabular}[c]{@{}c@{}}Optimized\\MSR\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Learned\\MSR\end{tabular}} \\ \cline{2-7} 
    \multicolumn{1}{r|}{TMQI$\uparrow$}  & \multicolumn{1}{c|}{\textbf{0.951}}   & \multicolumn{1}{c|}{0.809}  & \multicolumn{1}{c|}{0.850}  & \multicolumn{1}{c||}{0.866} & \multicolumn{1}{c|}{0.923}  & \multicolumn{1}{c|}{0.934} \\ \cline{2-7} 
    \multicolumn{1}{r|}{Underexposure$\downarrow$} & \multicolumn{1}{c|}{\textbf{0.535}}    & \multicolumn{1}{c|}{0.755}  & \multicolumn{1}{c|}{2.842} & \multicolumn{1}{c||}{1.191}   & \multicolumn{1}{c|}{1.803}  & \multicolumn{1}{c|}{1.330}  \\ \cline{2-7} 
    \multicolumn{1}{r|}{Overexposure$\downarrow$}  & \multicolumn{1}{c|}{0.899}    & \multicolumn{1}{c|}{1.628}  & \multicolumn{1}{c|}{\textbf{0.030}}   & \multicolumn{1}{c||}{1.578} & \multicolumn{1}{c|}{1.176}    & \multicolumn{1}{c|}{1.110} \\ \cline{2-7} 
    \multicolumn{1}{r|}{Loss of Global Contrast$\downarrow$}  & \multicolumn{1}{c|}{-0.162}   & \multicolumn{1}{c|}{-0.123} & \multicolumn{1}{c|}{-0.084}   & \multicolumn{1}{c||}{-0.148}  & \multicolumn{1}{c|}{\textbf{-0.202}}   & \multicolumn{1}{c|}{-0.152} \\ \cline{2-7} 
    \multicolumn{1}{r|}{Loss of Local Contrast$\downarrow$}    & \multicolumn{1}{c|}{-0.041} & \multicolumn{1}{c|}{-0.024} & \multicolumn{1}{c|}{-0.022}   & \multicolumn{1}{c||}{-0.027}   & \multicolumn{1}{c|}{\textbf{-0.044}}  & \multicolumn{1}{c|}{-0.031} \\ \cline{2-7} 
    \multicolumn{1}{r|}{Noise Visibility$\downarrow$}  & \multicolumn{1}{c|}{-}                 & \multicolumn{1}{c|}{30.77}   & \multicolumn{1}{c|}{30.04}  & \multicolumn{1}{c||}{28.79}   & \multicolumn{1}{c|}{30.67}  & \multicolumn{1}{c|}{\textbf{26.49}}  \\ \cline{2-7} 
    \multicolumn{1}{r|}{Global Temporal Incoherence$\downarrow$} & \multicolumn{1}{c|}{$1.7\text{e}^{-4}$}  & \multicolumn{1}{c|}{$3.7\text{e}^{-4}$} & \multicolumn{1}{c|}{$2.8\text{e}^{-5}$} & \multicolumn{1}{c||}{$2.7\text{e}^{-4}$}   & \multicolumn{1}{c|}{$2\text{e}^{-5}$}   & \multicolumn{1}{c|}{\textbf{$\mathbf{5.7e^{-6}}$}} \\ \cline{2-7} 
    \multicolumn{1}{r|}{Local Temporal Incoherence$\downarrow$} & \multicolumn{1}{c|}{\textbf{0.0048}}  & \multicolumn{1}{c|}{0.0157} & \multicolumn{1}{c|}{0.0088} & \multicolumn{1}{c||}{0.0394}  & \multicolumn{1}{c|}{0.025}  & \multicolumn{1}{c|}{0.0258}  \\ \cline{2-7} 
    \end{tabular}
  %  }
    \label{tab:Final_comparison}
\end{table}

==> Joint tone mapping and denoising of thermal infrared images via multi-scale Retinex and multi-task learning/tables/Retinex_optimizations_noHistMatch.tex <==
\begin{table}[ht]
    \caption{Comparison between the state-of-the-art \acp{TMO} and the baseline \ac{MSR} algorithm with different optimizations. The proposed optimized \ac{MSR} performs best among the Retinex-based algorithms especially for the \ac{TMQI} measure.}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{rccccccc}
    \multicolumn{1}{c}{\textbf{}}                    & \textbf{FLIR~\cite{FLIR_dataset}}                       & \textbf{\begin{tabular}[c]{@{}c@{}}Realtime~\cite{Eilertsen2015}\\TMO\end{tabular}} & \textbf{\ac{CGF}~\cite{Haibo_conditional_filtering_MSR}} & \textbf{\ac{MSR}\cite{Petro2014}} & \textbf{\begin{tabular}[c]{@{}c@{}}\ac{MSR}+\\CLAHE\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\ac{MSR}+\\Sigma\\Clipping\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Optimized\\\ac{MSR}\end{tabular}} \\ \cline{2-8} 
    \multicolumn{1}{r|}{TMQI$\uparrow$}                        & \multicolumn{1}{c|}{\textbf{0.951}} & \multicolumn{1}{c|}{0.809}  & \multicolumn{1}{c|}{0.850}         & \multicolumn{1}{c|}{0.866}                                      & \multicolumn{1}{c|}{0.887}                                                                                         & \multicolumn{1}{c|}{0.921}           & \multicolumn{1}{c|}{0.923}                                           \\ \cline{2-8} 
    \multicolumn{1}{r|}{Underexposure$\downarrow$}               & \multicolumn{1}{c|}{\textbf{0.535}}          & \multicolumn{1}{c|}{0.755}  & \multicolumn{1}{c|}{2.842}   & \multicolumn{1}{c|}{1.191}                                      & \multicolumn{1}{c|}{1.212}                                                                         & \multicolumn{1}{c|}{1.685}                  & \multicolumn{1}{c|}{1.803}                         \\ \cline{2-8} 
    \multicolumn{1}{r|}{Overexposure$\downarrow$}                & \multicolumn{1}{c|}{0.899}          & \multicolumn{1}{c|}{1.628} & \multicolumn{1}{c|}{\textbf{0.030}}   & \multicolumn{1}{c|}{1.580}                                      & \multicolumn{1}{c|}{2.437}                                                                       & \multicolumn{1}{c|}{0.860}                     & \multicolumn{1}{c|}{1.176}                                \\ \cline{2-8} 
    \multicolumn{1}{r|}{Loss of Global Contrast$\downarrow$}     & \multicolumn{1}{c|}{-0.162}         & \multicolumn{1}{c|}{-0.123}   & \multicolumn{1}{c|}{-0.084}   & \multicolumn{1}{c|}{-0.148}                                     & \multicolumn{1}{c|}{\textbf{-0.204}}               & \multicolumn{1}{c|}{-0.151}                       & \multicolumn{1}{c|}{-0.202}                              \\ \cline{2-8} 
    \multicolumn{1}{r|}{Loss of Local Contrast$\downarrow$}      & \multicolumn{1}{c|}{-0.0417}        & \multicolumn{1}{c|}{-0.0233}  & \multicolumn{1}{c|}{-0.022}  & \multicolumn{1}{c|}{-0.0270}                                    & \multicolumn{1}{c|}{-0.0425}               & \multicolumn{1}{c|}{-0.0290}                   & \multicolumn{1}{c|}{\textbf{-0.0447}}                                 \\ \cline{2-8} 
    \multicolumn{1}{r|}{Noise Visibility$\downarrow$}            & \multicolumn{1}{c|}{-}              & \multicolumn{1}{c|}{30.77}  & \multicolumn{1}{c|}{30.04}    & \multicolumn{1}{c|}{\textbf{28.79}}                                      & \multicolumn{1}{c|}{30.61}                                     & \multicolumn{1}{c|}{29.50}                            & \multicolumn{1}{c|}{30.67}                          \\ \cline{2-8} 
    \multicolumn{1}{r|}{Global Temporal Incoherence$\downarrow$} & \multicolumn{1}{c|}{$1.7\text{e}^{-4}$}       & \multicolumn{1}{c|}{$3.6\text{e}^{-4}$}  & \multicolumn{1}{c|}{$2.8\text{e}^{-5}$}  & \multicolumn{1}{c|}{$2.7\text{e}^{-4}$}                                   & \multicolumn{1}{c|}{$1.5\text{e}^{-4}$}               & \multicolumn{1}{c|}{$\mathbf{1.6e^{-5}}$}                      & \multicolumn{1}{c|}{$2\text{e}^{-5}$}                              \\ \cline{2-8} 
    \multicolumn{1}{r|}{Local Temporal Incoherence$\downarrow$}  & \multicolumn{1}{c|}{\textbf{0.0048}}        & \multicolumn{1}{c|}{0.0158} & \multicolumn{1}{c|}{0.0088} & \multicolumn{1}{c|}{0.0394}                                     & \multicolumn{1}{c|}{0.0253}                                                                        & \multicolumn{1}{c|}{0.0389}                      & \multicolumn{1}{c|}{0.025}                               \\ \cline{2-8} 
    \end{tabular}
    }
    \label{tab:Retinex_optimization}
\end{table}
